Into the Unknown: Assigning Reviewers to Papers with Uncertain Affinities

A successful peer review process requires that qualified and interested reviewers are assigned to each paper. Most automated reviewer assignment approaches estimate a real-valued affinity score for each paper-reviewer pair that acts as a proxy for the quality of the match, and then assign reviewers to maximize the sum of affinity scores. Most affinity score estimation methods are inherently noisy: reviewers can only bid on a small number of papers, and textual similarity models and subject-area matching are inherently noisy estimators. Current paper assignment systems are not designed to rigorously handle noise in the peer-review matching market. In this work, we assume paper-reviewer affinity scores are located in or near a high-probability region called an uncertainty set. We maximize the worst-case sum of scores for a reviewer assignment over the uncertainty set. We demonstrate how to robustly maximize the sum of scores across various classes of uncertainty sets, avoiding potentially serious mistakes in assignment. Our general approach can be used to integrate a large variety of paper-reviewer affinity models into reviewer assignment, opening the door to a much more robust peer review process.

==> figs/welfarevaryingalpha.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{../figs/WelfareVaryingAlpha.png}
    \caption{Ground-truth and worst-case welfare for TPMS algorithm vs. Robust Maximin Allocation on datasets derived from the MIDL conference data. $1-\alpha$ indicates the concentration of noise on the paper-reviewer pairs assigned by the TPMS allocation, so $\alpha=0$ concentrates all noise on the pairs assigned by TPMS, and $\alpha=1$ concentrates all noise on pairs not assigned by TPMS. \justin{I think we want to re-run this with the updated algorithm.}}
    \label{fig:welfarevaryingalpha}
\end{figure}


==> tables/iclr_baselines.tex <==

\begin{table*}
      \centering
        \caption{Adversarial and average-case $\USW$ for
        %three
        $3$
        baselines on $5$ recent ICLR conferences. Means and standard deviations
        %for each entry
        are reported over $100$ repetitions of sampling $60\%$ of reviewers and papers for each conference year.}
        \renewcommand{\toprule}{\hline}
        \renewcommand{\midrule}{\hline}
        \renewcommand{\bottomrule}{\hline}
        % \renewcommand{\arraystretch}{2.25}
        \setlength{\tabcolsep}{0.5em} % for the horizontal padding
        \renewcommand{\arraystretch}{1.0}% for the vertical padding

        \begin{tabular}{c||ccc|ccc}
        %\begin{tabularx}{\linewidth}{ccc|rrrr}
            \toprule
            \multirow{2}{*}{\textbf{Year}} & \multicolumn{3}{c|}{\textbf{Adversarial USW}} & \multicolumn{3}{c}{\textbf{Average USW}} \\
            & \textbf{FairFlow} & \textbf{PR4A } & \textbf{FairSeq } & \textbf{FairFlow } & \textbf{PR4A } & \textbf{FairSeq }\\
            \toprule            
            $2018$ & $0.072 \pm 0.027$ & $0.166 \pm 0.028$ & $0.159 \pm 0.027$ & $1.343 \pm 0.117$ & $1.772 \pm 0.017$ & $1.769 \pm 0.022$ \\
            
            $2019$ & $0.122 \pm 0.022$ & $0.220 \pm 0.022$ & $0.217 \pm 0.022$ & $1.391 \pm 0.089$ & $1.835 \pm 0.013$ & $1.832 \pm 0.013$ \\
            $2020$ & $0.109 \pm 0.020$ & $0.175 \pm 0.016$ & $0.172 \pm 0.015$ & $1.583 \pm 0.079$ & $1.867 \pm 0.011$ & $1.864 \pm 0.011$ \\
            $2021$ & $0.183 \pm 0.015$ & $0.233 \pm 0.017$ & $0.230 \pm 0.016$ & $1.770 \pm 0.021$ & $1.916 \pm 0.011$ & $1.913 \pm 0.011$ \\
            $2022$ & $0.225 \pm 0.016$ & $0.275 \pm 0.017$ & $0.274 \pm 0.016$ & $1.770 \pm 0.007$ & $1.901 \pm 0.010$ & $1.899 \pm 0.010$ \\
            \bottomrule
%\end{tabularx}
\end{tabular}
\label{tab:baselines_iclr}
\end{table*}

==> tables/iclr_basic_stats.tex <==

\begin{table}
      \centering
        \caption{Number of reviewers and papers for each year of ICLR.}
        \begin{tabularx}{\linewidth}{XXX}
            \toprule
            Year & Reviewers & Papers \\
            \toprule
            $2018$ & $2762$ & $911$ \\ 
            \midrule
            $2019$ & $4367$ & $1419$ \\
            \midrule
            $2020$ & $6872$ & $2213$ \\
            \midrule
            $2021$ & $7770$ & $2595$ \\
            \midrule
            $2022$ & $8372$ & $2627$ \\
            \bottomrule
\end{tabularx}
\label{tab:iclr_basic_stats}
\end{table}

==> tex/ethical.tex <==
\section*{Ethical Statement}

% Our approach does not consider fairness to papers, which has been incorporated in a few prior works. 
Our suggestions to build models of downstream review quality may result in models that disadvantage certain types of papers or reviewers --- for example, models may be poor at predicting downstream review quality for papers in a less popular domain. 
However, we expect that introducing fairness objectives into the optimization problem would mitigate unfairness due to poorer predictions from such models. Any changes in the review process should be undertaken with caution and additional testing, as small changes in the algorithm can drastically affect some authors' and reviewers' experiences. 
